Guarding Polygons with Holes

We study the Cooperative Guarding problem for polygons with holes in a mobile multi-agents setting. Given a set of agents, initially deployed at a point in a polygon with $n$ vertices and $h$ holes, we require the agents to collaboratively explore and position themselves in such a way that every point in the polygon is visible to at least one agent and that the set of agents are visibly connected. We study the problem under two models of computation, one in which the agents can compute exact distances and angles between two points in its visibility, and one in which agents can only compare distances and angles. In the stronger model, we provide a deterministic $O(n)$ round algorithm to compute such a cooperative guard set while not requiring more than $\frac{n + h}{2}$ agents and $O(\log n)$ bits of persistent memory per agent. In the weaker model, we provide an $O(n^4)$ round algorithm, that does not require more than $\frac{n+2h}{2}$ agents.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file


==> ba_conclusion.tex <==
% !TEX root = main.tex

\section{Conclusion and Future Works}

% In this paper, we have studied the Cooperative Guards from a distributed mobile agent perspective. We studied two different models where agents had different sensing capabilities. In one model, which we call the {\it depth perception} model, the agents are able to entirely map out the polygon by estimating co-ordinates. The second model, which we call the {\it proximity perception} model, the agents have limited sensing capabilities. We compare the difficulties of solving the problem in the two models, providing efficient linear time algorithms in the stronger model and a polynomial ($O(n^4)$) time algorithm in the weaker model. \onlyLong{In the stronger model, we provide multiple algorithms that run in linear number of rounds, that trade-off between the number of broadcasts performed, the amount of information sent in a single round and the number of guards placed.}
We discuss about further improvements and some closely related open problems below.

\textbf{Open Problem 1. } {\em {How many co-operative guards are required for a polygon with $n$ vertices and $h$ holes?  What if guards are restricted to be on the vertices of the polygon? }} 
We gave a construction that required $\frac{n + h - 2}{2}$ co-operative guards, however we have not been able to construct polygons requiring so many guards. For $h \leq 1$, the problem has been solved by Zylinski \cite{zylinski2005cooperative}, but for $h \geq 2$, the problem remains open. We have not been able to provide a better upper bound than $\frac{n + 2h - 2}{2}$ guards when the guards are restricted to the vertices of the polygon. We have also not been able to construct polygons where the number of {\em vertex guards} required is more than $\frac{n + h - 2}{2}$, so we believe that there might exist a way to place $\frac{n + h - 2}{2}$ guards, by placing them only on the vertices of the polygon.

\textbf{Open Problem 2. } {\em {Is there a more efficient centralized algorithm to compute a cooperative guard set with $\frac{n + h - 2}{2}$ guards?}}
The centralized algorithm proposed runs in $O(n^2)$ time, whereas we are able to construct a cooperative guard set using no more than $\frac{n + 2h - 2}{2}$ agents in $O(n \log n)$ time. Is it possible to bridge the gap in the running time? One possible approach might be to construct the reduction proposed by Sachs and Souvaine~\cite{BjorlingSachs1995} by using a divide and conquer algorithm on the holes.

\textbf{Open Problem 3.} {\em {Is it possible to construct $O(poly(D))$ time algorithms where $D$ is the hop diameter of the polygon, when agents have limited persistent memory? }}
The hop diameter of the polygon is the minimum number of straight line segments required to connect any two vertices of the polygon. In simple polygons, it is easy to construct such algorithms. However in polygons with holes, if the agents split up at any point for exploration, we could end up in a situation where two guards are symmetric with respect to each other. We suspect that randomization might help, though it is not clear to us, whether it is even possible when the agents are deterministic.

% \textbf{Open Problem 4.} {\em {Gathering in Polygons. Is it possible to efficiently gather a group of agents all located in a polygon (but not necessarily visibly connected)?}}

% Our exploration algorithms rely on the fact that the agents all start in a single location. Thus, an algorithm that can gather all the agents could be used as a pre-processing step to remove this restriction. In the case when the agents have limited memory, it is not clear to us how to gather them efficiently.


==> ba_intro.tex <==
% !TEX root = main.tex

\section{Introduction}
% \enlargethispage{\baselineskip}

The {\it Art Gallery Problem} is a classical computational geometry problem which asks for the minimum number of guards required to completely guard the interior of a given art gallery. 
The art gallery is modelled as a simple polygon and guards are points on or inside the polygon. 
A set of guards is said to guard the art gallery, if every point in the art gallery is visible to at least one guard. 
% This problem was first posed by Klee in 1973, and has since been well studied over the years (see 
% \cite{O'Rourke:1987:AGT:40599,163407,URRUTIA2000973,G07}). 
This problem was first posed by Klee in 1973 and since then the problem has been of interest to researchers. 
The problem and its many variations have been well-studied over the years. Chv\'{a}tal \cite{CHVATAL197539} was the first to show that $\lfloor \frac{n}{3} \rfloor$ guards are sufficient and sometimes necessary to guard a polygon with $n$ vertices. 
Fisk \cite{FISK1978374} proved the same result via an elegant coloring argument, which also leads to an $O(n)$ algorithm that computes such a guard set. 
% The problem of finding the minimum number of guards was shown to be NP-hard (Lee and Lin \cite{1057165}) as well as APX-hard(Eidenbenz {\it et al.}\cite{Eidenbenz2001}). 
% Consequently, researchers have focussed on approximation algorithms (Ghosh~\cite{G87}, Deshpande {\it et al.} \cite{deshpande2007pseudopolynomial},  and Bhattacharya {\it et al.} ~\cite{BGP17}).

% Popular variants of the $\{it Art Gallery Problem}$ are the $\it{orthogonal Art Gallery Problem}$ in which all interior angles in the 
% polygon are either 90 or 270. 

% \st{In this paper, }
We study a variant of the classical Art Gallery Problem known as the {\em Cooperative Guards} problem in polygons with holes from a distributed multi-agents perspective. 
The {\em Cooperative Guards} problem is similar to the {\it Art Gallery Problem} with the additional constraint that the visibility graph of the guards, i.e., the graph with guards as vertices and edges between guards that can see each other, should form a single connected component. 
This implies that if the guards can communicate through line of sight, then any two guards can communicate with each other (either directly or indirectly through intermediate guards). 
The {\it Cooperative Guards} problem was first introduced by Liaw {\it et al.} in 1993 ~\cite{Liaw1993TheMC}, in which they show that this variant of the {\it Art Gallery Problem} is also NP-hard.

The pursuit of solving the {\it Cooperative Guards} problem for us is primarily motivated by the search for distributed multi-agent exploration algorithms for agents deployed in the polygon. 
One of the easiest ways to explore the polygon is by maintaining connectivity through line of sight and having the agents cooperatively send exploratory agents and expand the area of the polygon that they can collectively see. Such an algorithm would require the agents to be visibly connected and if at the end they are collectively able to see the entire polygon, then they form a solution to the {\it Cooperative Guards} problem. 
This lead us to first tackle the {\it Cooperative Guards} problem in the centralized setting and adapt it to the distributed multi-agent model. 
Note that once the agents are positioned to cooperatively guard the polygon, they can collectively solve \textit{any} computational geometry problem on the polygon by executing a distributed algorithm on their visibility graph. 
Hence our algorithm can also serve as an initial pre-processing step for distributed multi-agents to solve other problems on the polygon, for example they can compute the number of vertices of the polygon, diameter of the polygon etc. 
Our focus throughout this paper is to find time optimal algorithms for computing a set of cooperative guards on the polygon (not necessarily minimum). 
Analogous to Fisk's \cite{FISK1978374} coloring argument for the classical {\it Art Gallery Problem}, we provide an efficient algorithm that computes a set of visibly connected guards using no more than $\frac{n + h - 2}{2}$ guards. \\

\onlyLong{\subsection{Our Contributions}}
\onlyShort{\noindent {\bf Our Contributions.}}
Our goal is to design efficient deterministic algorithms for placing  cooperative guards in polygons with holes. While we warmup with a centralized algorithm, our main focus is on constructing distributed algorithms executed by mobile agents.

% \st{In Section~\ref{warmup} }
We first present a centralized algorithm for the Cooperative Guards problem in polygonal region with $n$ vertices and $h$ holes, that does not require more than $\frac{n+2h-2}{2}$ guards.
The centralized algorithm presented here runs in time $O(n+T(n, h))$ where $T(n, h)$ is the time required to triangulate a polygon with $n$ vertices and $h$ holes, i.e. after the initial step of triangulating the polygon, the algorithm takes linear time and places no more than $\frac{n + 2h - 2}{2}$ guards. 
We then use an observation from Zylinski \cite{zylinski2005cooperative} to reduce the number of guards to $\frac{n+h-2}{2}$. The reduction is slower and runs in $O(n^2)$ time.
% Zylinski \cite{zylinski2005cooperative} also shows that a better upper bound of $\frac{n + h - 1}{2}$ guards can be obtained 
% (refer Corollory 4.3), however it runs in $O(n^2)$ time. 

% In Section~\ref{model} 
We propose two distributed models of computation, one in which the agents can perceive exact distances (which we call {\em depth perception}) and hence can compute co-ordinates (with respect to some common reference frame) to map out the polygon, and another in which the agents receive only a combinatorial view of their visibility.  

% In Section~\ref{sec:algorithm} 
We present a distributed algorithm (in the stronger {\em depth perception} model) that runs in $O(n)$ rounds and does not require more than $\lfloor \frac{n + h - 2}{2} \rfloor$ agents. Our distributed algorithm emulates the centralized algorithms presented except that the polygon is not known in advance. We simultaneously explore and incrementally construct a  triangulation. 

% In Section~\ref{sec:algorithm:proximity} 
Finally, we present a distributed algorithm for the weaker {\em proximity perception } model, which takes $O(n^4)$ rounds, but requires $\frac{n+2h-2}{2}$ agents. 

A summary of the results is presented in Table \ref{tab:results}. 
% \onlyShort{Due to limited space, we have deferred some details (proofs and pseudocode) to the full version in the Appendix.}\\

% \john{Section 5 should be explicitly represented.}\john{Include a table with all the results.} \sri{Mentioned Section 5 and the table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%         Algorithm & Round Complexity & Broadcast Complexity & Persistent Memory & Guards  \\
%         \hline
%         1 & $O(n)$ & $O(n)$ & $O(n \log n)$ & $(n+h-2)/2$\\
%         2 & $O(n)$ & $O(n^2)$ & $O(\log n)$ & $(n+2h-2)/2$\\
%         3 & $O(n)$ & $O(n \log n)$ & $O(\log n)$ & $(n+2h-2)/2$\\
%         4 & $O(n)$ & $O(n (h + \log n))$ & $O(\log n)$ & $(n+h-2)/2$\\
%         5 & $O(n^4)$ & $O(n^4)$ & $O(\log n)$ & $(n+2h-2)/2$\\ 
%     \end{tabular}
%     \caption{Results}
%     \label{tab:results}
% \end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Model \& Algorithm & Rounds & Broadcasts & Persistent Memory & Guards  \\
        \hline
        Depth Perception & $O(n)$ & $O(n)$ & $O(n \log n)$ & $(n+h-2)/2$\\
        (Large memory) & & & & \\
        \hline
        Depth Perception & $O(n)$ & $O(n \log n)$ & $O(\log n)$ & $(n+2h-2)/2$\\
        (Small memory) & & & & \\
        \hline
        Depth Perception & $O(n)$ & $O(n (h + \log n))$& $O(\log n)$ & $(n+h-2)/2$\\
        (Improving guards) & & & & \\
        \hline 
        Proximity Perception & $O(n^4)$ & $O(n^4)$& $O(\log n)$ & $(n+2h-2)/2$\\ 
        \hline
    \end{tabular}
    \caption{A summary of our results with respective theorem numbers indicated in the first column.}
    \label{tab:results}
\end{table}

% The running time of the algorithm is an improvement over the algorithm presented by Obermeyer {\it et al.} \cite{OGB11} which takes $O(n^2)$ rounds in the worst case and the algorithm presented by Ashok {\it et al.}\cite{Bharat2020} which works only for simple polygons (without holes). Moreover, \cite{Bharat2020} requires upto $n$ agents to explore the polygon as a pre-processing step. 
% The total number of broadcasts performed by our algorithm is $O(n (\log n + h))$ and each broadcast has a size of {$O(\log \frac{n}{\epsilon})$ bits}), where $\epsilon$ is a parameter we use for modelling the precision with agents store the co-ordinates with respect to some reference frame. Apart from computing the visibility polygon, the agents on average require only $O(\log \frac{n}{\epsilon})$ bits of memory. In contrast, the algorithms by Obermeyer {\it et al.} \cite{OGB11} require $O(n \log n)$ bits on average and the size of the messages that can be sent in a single round is $O(n)$.

% \onlyLong{\subsection{Related Work}}
% \onlyShort{\noindent {\bf Related Work.}}
% Most of the algorithms developed for solving the {\it Art Gallery Problem} and its variants triangulate the polygon in the first step. 
% So we first look at the best known algorithms for triangulation.
% Chazelle \cite{Chazelle1991} provided a linear time algorithm for computing the triangulation of a simple polygon with $n$ vertices, however the algorithm is known to be quite complicated. 
% Simpler $O(n \log n)$ algorithms were established long before by Gary {\it et al.} \cite{garey1978triangulating}. For polygons with holes the algorithm by Bar-Yehuda and Chazelle \cite{BARYEHUDA1994} can be used to obtain an $O(n + h \log^{1 + \epsilon} h)$ time algorithm. 
% For polygons with holes the triangulation problem has an $\Omega(n \log n)$ lower bound (as shown by Asano {\it et al.}~\cite{ASANO1986221}). 
% Our algorithm involves triangulation as the first (and most time consuming) step and thus the run time of all algorithms is at best $O(n \log n)$ and slightly better when $h = o(n)$ if Bar-Yehuda and Chazelle's\cite{BARYEHUDA1994} algorithm is used. 

% Chv\'{a}tal \cite{CHVATAL197539} and Fisk \cite{FISK1978374} independently proved that $\lfloor \frac{n}{3} \rfloor$ guards are always sufficient and occasionally necessary to guard a simple polygon with $n$ vertices, with the latter providing an elegant constructive proof which can construct the desired set of guards in linear time.

% The classical {\it Art Gallery Problem} for polygons with holes was first solved by Souvaine {\it et al.} \cite{BjorlingSachs1995}. 
% They show that $\frac{n + h}{3}$ guards are sufficient (by presenting an $O(n^2)$ time algorithm) and sometimes necessary to guard a polygonal region with $n$ vertices and $h$ holes. 
% %They also provide an algorithm that computes such a guard set in $O(n^2)$. 

% The {\it cooperative guards} problem was first posed by Liaw \cite{Liaw1993TheMC} where they provide a solution for $k-$spiral polygons and also show that the problem is NP-hard. 
% Ahlfeld and Hecker \cite{AhlfeldUweandHecker92} were the first to prove that for simple polygons $\lfloor \frac{n-2}{2} \rfloor$ guards are sufficient and sometimes necessary. 
% Their algorithm relies on analysing the length of the longest degree $2$ chains in the dual graph. The dual graph is a graph corresponding to a triangulation of the polygon. 
% The vertices of the polygon correspond to a triangle in the triangulation and an edge is present between two vertices if their corresponding triangles share a common edge. 
% Hernandez-Penalver \cite{hernandez1994controlling} proved the same result by induction on the dual graph.
% Pinciu \cite{Pinciu} also provided an alternate proof of the same result by extending Fisk's coloring argument. Zylinski \cite{zylinski2007cooperative} also provided an alternate soluton based on the diagonal graph. 
% The diagonal graph is the graph induced by the diagonals of the triangulation. 
% A vertex cover of the diagonal graph gives a cooperative guard set with no more than $\lfloor \frac{n}{2} \rfloor$ guards. 

% For polygons with holes, Ahlfeld and Hecker \cite{AhlfeldUweandHecker92} were the first to show that $\lfloor \frac{n + 2h - 2}{2} \rfloor$ guards are sufficient, however the bound is not tight. 
% Zylinski \cite{zylinski2005cooperative} showed that for polygons with one hole, $\lfloor \frac{n-1}{2} \rfloor$ guards are sufficient and sometimes necessary.
% Zylinski \cite{zylinski2007cooperative} provided a better upper bound of $\frac{n + h - 1}{2}$ guards using ideas established by Sachs and Souvaine \cite{BjorlingSachs1995} that leads to an $O(n^2)$ algorithm. 
% Zylinksi \cite{zylinski2005cooperative} also provides a different linear time algorithm that takes no more than $\lfloor \frac{n + 2h - 2}{2} \rfloor$ guards.
% Zylinksi's book \cite{zylinski2007cooperative} contains a more extensive survey of these algorithms.

% The {\it Cooperative Guards} problem was first studied in the mobile-agents setting by Obermeyer {\it et al.} \cite{OGB11}. 
% Ashok {\it et al.}\cite{Bharat2020} provides a better $O(\min(D^2, n))$ time algorithm where $D$ is the maximum hop distance between any two points in the polygon, however it does not extend to polygons with holes and requires upto $n$ agents for exploration.

% In the mobile agents setting, several models have been proposed and studied over the years. A survey of such models is available in~\cite{DCME_book}. In most of them, the agents operate either on a graph or on the 2D-plane without obstacles or bounding structures. 

% In all the models studied in this paper, the movement of the agents is on a region of the 2D-plane that is bounded by a polygon (possibly with holes) that is not known in advance.  Consequently we need to learn and contend with the geometric complexities of the polygon to solve problems in our model(s).  There have been a few papers on mobile agents operating within bounded simple polygons (Ashok {\em et al.}~\cite{Bharat2020}). To the best of our knowledge, the only other work on mobile agents operating on a polygon with holes is by Obermeyer {\em et al.}~\cite{OGB11}. They provide an algorithm that takes no requires no more than $\lfloor \frac{n + 2h - 1}{2} \rfloor$ agents to collectively explore the polygon and deploy the agents so that they cooperatively guard the polygon. The running time of their algorithm is $O(n^2)$ rounds in the worst case. 


